A Survey and Perspective on Artificial Intelligence for Security-Aware Electronic Design Automation

Artificial intelligence (AI) and machine learning (ML) techniques have been increasingly used in several fields to improve performance and the level of automation. In recent years, this use has exponentially increased due to the advancement of high-performance computing and the ever increasing size of data. One of such fields is that of hardware design; specifically the design of digital and analog integrated circuits~(ICs), where AI/ ML techniques have been extensively used to address ever-increasing design complexity, aggressive time-to-market, and the growing number of ubiquitous interconnected devices (IoT). However, the security concerns and issues related to IC design have been highly overlooked. In this paper, we summarize the state-of-the-art in AL/ML for circuit design/optimization, security and engineering challenges, research in security-aware CAD/EDA, and future research directions and needs for using AI/ML for security-aware circuit design.

==> Sections/digital.tex <==
\subsection{Electronic Design Automation}\label{sec:eda}
The electronic design automation flow for digital ICs is as follows:

%Add EDA flow diagram: 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \subsubsection{Design Specification}
    In design specification, the designer must accurately describe the overall design requirements. The system may be proposed by a design team to initiate the production of a chip. The IC designers decide on functionality and plan out verification and testing procedures for the entire process.
    
\subsubsection{High-Level Synthesis}
    High-Level Synthesis (HLS) tools translate a design written in high-level languages such as C/C++/SystemC into a low-level hardware description language (HDL). Hardware components can be modeled at high levels of abstraction, allowing the designer to map both hardware and software components~\cite{martin_scheffer_lavagno_2016}
    
\subsubsection{Logic Synthesis}
     Logic synthesis is a direct translation from the behavioral domain (register transfer level) to the structural domain (gate level)~\cite{JIANG2009299}. The gate-level netlist is mapped to the standard cell library. The optimization part of logic synthesis minimizes hardware by finding equivalent representations of larger blocks. Design constraints used as input may also be met for circuit area, power, and performance.
    

\subsubsection{Design for Testability (DFT)}
   DFT encompasses the techniques used to generate cost-effective tests for the gate-level netlist obtained from logic synthesis. These techniques are geared towards increasing observability, controllability, and predictability of the design~\cite{martin_scheffer_lavagno_2016}. Ad-hoc methods like partitioning and test point insertion are relatively easier to implement, while structured ones like scan registers, scan chains, scan architectures and algorithms ensure good testability at the expense of additional area and delay overhead. The resulting tests utilize test programs which drive automatic test equipment (ATE). The ATEs also use automatic test pattern generation (ATPG) to identify input sequences which trigger errant circuit behavior arising from manufacturing defects~\cite{HSIAO2006161}. 

     
\subsubsection{Floorplanning}
    Flooplanning focuses on the sizes and arrangement of the physical blocks created during logic synthesis. It affects the optimization results of the increasing physical stages. It is the first major step in physical design. Pins and ports are also assigned a rough location, which can further be refined depending on the placement and routing results~\cite{Lienig2020}.

    
\subsubsection{Placement-and-Routing}
   After a successfully-proposed floorplan, the place-and-route~(P\&R) addresses the structural design of a circuit. The designer places and connects all of the blocks that make up the chip such that they meet design criteria and constraints. After the initial P\&R attempts, the design's timing constraints are analyzed. If unsatisfactory, the P\&R software in use tries different placements and signal routing to try to meet the designated constraints~\cite{Lienig2020}.

\vspace{1em}



\subsection{General Security Applications at Various Stages of Electronic Design Automation}

ML is already applied to some extent in the digital IC design process, albeit with primary focus on general design prediction and optimization. Some needs tackled at this stage include logic and design optimization~\cite{Haaswijk2018}, low-power approximation~\cite{Pasandi2020} and area estimation~\cite{froemmer2020}. Careful assessment of available publications incorporating learning into digital IC design will reveal an absolute truth; very little work has been done to directly address hardware security vulnerabilities. The use of intelligent models presents the opportunity to not only optimize designs, but to secure them against the array of tools and attacks that malicious parties have at their disposal. This is especially important for some security properties that cannot be modelled analytically and situations where multiple security constraints are at odds. According to~\cite{huang2021machine}, ML approaches in EDA can be broken down into four main directions: \textbf{decision making}, \textbf{performance prediction}, \textbf{black box optimization or design space exploration} and \textbf{AI-assisted EDA}. In the rest of this section, we follow this same organization to discuss security-aware CAD research and opportunities. Fig.~\ref{fig:icsecurity} also highlights the general EDA steps and the applicable directions for each one.

The decision-making perspective encapsulates the replacement of traditional, brute-force design-for-security methods with more automated and efficient techniques. In most cases, brute-force techniques involve countless trial-and-error steps until the best-performing configuration is found and used on a design. From a heuristic perspective, the knowledge gained may prove to be invaluable. However, they are only feasible on simpler designs; increased complexity transforms them into cumbersome requirements that most designers would gladly bypass. Further, the tradeoffs between security and traditional metrics as well as between different security metrics might be unknown or too complex for manual tuning. Automation becomes valuable only when it is characterized by efficiency. ML can definitively make decisions on the most suitable settings and parameters for countermeasures with varying levels of human input~(see Fig.~\ref{fig:decisionmaking}).

Performance prediction describes forecasting and modeling trade-offs associated with adding countermeasures, especially at earlier design stages. Although an ideal scenario would involve achieving optimum design goals while guaranteeing near-perfect security awareness, a designer must be aware of the inevitable compromises that a secure design may entail. A more achievable target is finding the balance between optimization and security, as seen in Fig.~\ref{fig:performanceprediction}. This is where AI/ML comes into the picture. The automation of the balance-seeking process will not only speed up the IC design pipeline, but will ensure that the most suitable operating parameters and modifications are available to the designer. From a business standpoint, time-to-market of ICs in production may also decrease.

For design space exploration, AI/ML seeks the solution that best meets requirements from available choices with little to no human intervention. The expanse of the search space creates the need for automation to execute selection, generation and evaluation of the solutions. However, the exhaustive option may not always be the optimal one, regardless of the availability of automation techniques. Design space exploration employs the application of different methods: stochastic optimization methods, like random search, evolutionary algorithms and black box optimization~\cite{CARDOSO201799}. Black box optimization uses a set of configurable parameters as inputs instead of results from the design stages, as seen in Fig.~\ref{fig:blackbox}. The circuit may either be too complex to model, or the engineer lacks details of the design to work with. At the training stage, most ML/AI algorithms are being optimized to find the best fit for input parameters, constraints, and design features. Hence, finding the most suitable design based on specifications may be the most intuitive application to the digital IC design.



\begin{figure*}[t]
   \includegraphics[width=\textwidth]{Images/IC Design with Security Topics.png}
   \centering
   \caption{General digital IC design pipeline with applicable security topics for each stage. \textbf{D} stands for decision making, \textbf{P} represents performance prediction, while \textbf{B} and \textbf{A} stand for black box optimization or design space exploration and AI-assisted EDA, respectively.}
   \label{fig:icsecurity}
\end{figure*}
%Replace brute-force by automatically deciding which tools/scripts/steps to run or countermeasures to add during design
%Feature-based models especially for parameter selection of countermeasures

%\subsection{\textbf{Decision Making}}\label{subsection: decisionmaking}
\subsubsection{High Level Synthesis and/or Register Transfer Level}\label{sec: hlsrtl}
%Insert text?

%	E.g.) AISS @ HLS/RTL levels to choose primitives to deploy
\paragraph{\textbf{Hardware Security Primitive Deployment at Higher Levels of Abstraction}}\label{subsubsec: aiss}
The Automatic Implementation of Secure Silicon (AISS) program was developed by the Defense Advanced Research Projects Agency (DARPA) to automate the process of incorporating scalable defense mechanisms into chip designs, by allowing designers to explore chip economics versus security trade-offs based on the expected application and intent while maximizing designer productivity~\cite{darpa}. Deployment of security methods pre-silicon are always cost-effective and less time-consuming. With this in mind, AI/ML can be used to make decisions as early as during HLS, or at RTL. Based on the discernible features at these levels of abstraction, a classification-based model can use vector embeddings to suggest suitable hardware security primitives and their associated parameters (e.g., size). For example silicon odometers are inserted into IC designs to measure aging and detect recycled counterfeit chips~\cite{guin2015design}. Their accuracy and yield are determined by various parameters~\cite{shakya2015performance}, which can be optimized through ML/AI. 

Physically unclonable functions (PUFs)~\cite{gassend2002silicon} provide digital fingerprints using the internal process variations (entropy) of a physical device. The translation of these unique and unclonable manufacturing variations into challenge-response pairs provides unique chip identifiers or authentication mechanisms. One of the main issues with PUFs is their reliability,~\ie{} ability to provide the same output in the presence of environmental variations and aging. To combat this, they often rely on error correcting codes~\cite{hiller2020review}, which can be designed to handle a specific number of bit flips. Another primitive is the true random number generator (TRNG), which uses an entropy source to generate non-deterministic data with a given throughput to seed security algorithms like cipher keys~\cite{gabriel_wittmann_sych_dong_mauerer_andersen_marquardt_leuchs_2010} or masking~\cite{trichina2003combinational}. For any design that contains all three of these primitives, their characteristics can be tuned together for a specific application or to fit within a dedicated silicon area.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% E.g.) Encoding optimization: Use one hot encoding instead of binary encoding for more secure FSMs
\paragraph{\textbf{Encoding Optimization}}\label{subsubsec: encoding}
Another aspect that stands to benefit from the addition of ML-powered decision-making is finite state machine (FSM) encoding optimization. The encoding schemes are selected based on design constraints, including power and area. The two most common options are:

\begin{itemize}
\item \textbf{Binary Encoding} -
In binary encoding scheme, states are encoded as a binary sequence where the states are numbered starting from 0 and up. The number of state flip-flops (FFS), $q$, required for binary encoding scheme is given by $q = log2(n)$; where, $n$ is the number of states. The binary encoding scheme is better suited for FSM with a fewer number of states~\cite{lin2012binary}.

\item \textbf{One-hot Encoding} -
This encoding scheme is designed with only one bit of the state variable as ``1'' while all other state bits are ``0''. It requires as many state FFs as the number of states. This creates the need for more state FFs than binary encoding~\cite{cassel2006onehot}.
\end{itemize}

One-hot encoding scheme is less vulnerable to fault injection attacks while binary is more resistant to hardware Trojans that exploit don't care states. This is demonstrated by Nahiyan~\etal{} using the FSM of the SHA-256 digest engine~\cite{nahiyan2019}. With this knowledge, a secure encoding scheme was proposed in~\cite{nahiyan2019} that combines binary and one-hot schemes to achieve the best of both worlds. In future work, AI/ML may be used to determine the best mix given a specific FSM.
%A polynomial regression model can be trained to balance security awareness with reasonable overhead.


% •	E.g.) Creating (mask) gadgets Ask Dr. Forte for clarification- Side channel masking Ask Saba
\paragraph{\textbf{Crafting Side Channel-resilient Circuits}}
Referring to Section~\ref{subsubsec: sidechannelresist}, masking has been introduced to stop an attacker from mounting side channel analysis. 
AI has become an integral part of this, for instance, RL has been applied to combine a set of countermeasures, which leads to the enhancement of target resilience to, at least, some types of attacks \cite{rijsdijk2021reinforcement}. 
Seen from another perspective, machine learning algorithms, and in particular, NNs, can defeat some countermeasures, including masking~\cite{kim2019make,related_works:automated_hyperparameter_tuning,related_works:SCA_metrics}. 
As an example of such attacks, RL has been employed to determine proper side-channel leakage models and training of neural networks to extract leakage profiles~\cite{DBLP:journals/iacr/RijsdijkWPP21}.
Hence, robustness against such attacks has become one of the objectives of the tests conducted to evaluate the effectiveness of countermeasure, specifically, masking. 
%the efficacy of masking to sever the relationship between input/functionality and side channel information, specifically for cryptographic systems can be measured using ML. 

Given the nature of such tests, the security-aware designer may have to deal with the higher levels of abstraction corresponding to a black box leakage model because there is no information, including physical placement or routing signals \cite{buhan2021sok}.
Therefore, masking schemes may be implemented, but there is no guaranteed measure of effectiveness before the RTL stage.
To enhance this process, full access to the design's layout available to the implementing party could be useful and even be bolstered with an understanding of the device's functionality via RTL or gate-level implementation. 
This is in line with the studies focused on modeling the implementation and simulating its behavior as discussed before~\cite{bertoni2017methodology,reparaz2016detecting}. 
In this context, AI has not yet reached its full potential as security-critical implementations are still designed manually.  
The manual design and implementation pose a series of drawbacks stemming from (1) the lack of integration between the various designs, (2) erroneous designs due to human errors, and (3) high consumption of resources, including time (both execution and design times), silicon area and/or power/energy consumption. 


% •	E.g.) Predict Trojan detection rates (dummy scan FF insertion, assertions, BISA, Split Manufacturing, run-time methods)
\paragraph{\textbf{Hardware Trojan Detection Rates at Register Transfer Level}}
Malicious modifications,~\ie{} \textbf{hardware Trojans}, are possible during the IC design and fabrication process. Hardware Trojan detection has been extensively researched within the hardware security research domain~\cite{tehranipoor2010}. Salmani~\etal{} proposed a method of increasing the probability of Trojan activation using dummy scan FFs~\cite{salmani2012}. They place a dummy scan FF with a net having low transition probability. To test the concept, Trojan samples have to be deployed on benchmarks. The rate of Trojan detection could be derived from the available data that these simulations produce. Likely features that would be valuable for a prediction-based ML model include nets with dummy scan FFs, their fanouts and their corresponding transition probabilities. 

\textbf{Assertions} are typically used for formal verification of specification patterns. The behavior of circuits determines the correctness of the design. Alsaiari~\etal{} propose reconfigurable assertion checkers which are able to detect hardware Trojan updates on system-on-chips (SoCs)~\cite{alsaiari2019}. The design flow can be seen in Fig.~\ref{fig:assert}. Even with traditional assertion checkers where selection only occurs pre-synthesis, it is possible to ascertain the rate of Trojan detection using the assertion checkers, the Trojan type, as well as the point(s) of insertion.


\begin{figure}[t!]
\centering
%\includegraphics[width=0.85\columnwidth]{traceDefectsBorder.png}
\includegraphics[width=0.5\columnwidth]{Images/asserion checker paper.PNG}
\caption{Digital IC design flow with inserted assertion checkers. Reprinted from~ \cite{alsaiari2019}.}
\label{fig:assert}
\end{figure}



\subsubsection{Logic Synthesis}\label{sec:logicsynth}


\paragraph{\textbf{Tuning EDA Parameters and Commands during Logic Synthesis}}\label{subsubsec: dectuninglogic}
%\paragraph{Logic Synthesis}\label{par: dectuning, logic}
%One realistic instance is tuning timing, power and area constraints provided at the logic synthesis stage.
Although a constraint set may be part of the design specification, the gate level netlist provides a better understanding of functionality to a designer. Area constraints guide the P\&R tool to locate a specified design block partition, while timing constraints specify path delays~\cite{else2009}. To tune high-level directives, it is important to accurately predict their impact. This is a tall order for most designs due to complex optimizations throughout the design process. These complex optimizations create disparity between desired results at the HLS stage and implemented values post-synthesis. Conventional tools assist with optimization tasks, but machine learning is already being used to mitigate the latter problem. For example, Yu~\etal{}~\cite{yu2018developing} have developed Intellectual Property (IP)-specific synthesis flows (i.e., sequence of synthesis transformations for TCL scripts) using CNNs that improve Quality of Result (QoR). In~\cite{Neto2019LSOracleAL}, DL is used to automatically decide which logic optimizer (And-Inverter Graph (AIG) and Majority-Inverter Graph (MIG)) should handle different portions of the circuit for better performance and lower area. Makrani~\etal{}~\cite{Makrani2019} proposed a Pyramid framework to estimate best performance and resource usage. The input features are derived from the HLS report, and a stacked regression model provides accurate timing, delay and resource values before reaching post-implementation. 

Optimization goals during tuning can be geared towards obtaining a more secure, synthesised design with minimum overhead. Although this would only be evident with the combination of other design parts, early-stage deployment saves time and labor. For example, secure split-test (SST) is a method of securing the manufacturing process by mandating test results to be verified by the IP owner and by using a ``key'' to unlock the IPs correct functionality after tests are passed. For the functional locking block, XOR logic is added in series to non-critical paths. If the two inputs are different, the XOR logic will act as an inverter~\cite{contreras2013} causing any locked (still untested or failed chip) to act deliberately incorrect. The optimal number of XOR gates to insert into the circuit, insertion algorithm~\cite{chakraborty2009harpoon,6616532,lee2015improving}, or partitioning algorithm~\cite{alaql2021saro} to employ for a given IP's function and/or structure can be determined using ML techniques. 




\paragraph{\textbf{Standard Cell Selection}}\label{subsubsec: standardcell} A specific category of available standard cells may be used in an IC design to address specific security vulnerabilities. As far back as 2004, sleep transistor cells were proposed as a method for sub-threshold leakage current reduction~\cite{babighian2004}. The sleep transistor cells are picked from a library designed to target high layout efficiency. The results were shown to have achieved a minimum reduction percentage of 74\%. A trained support vector machine~(SVM) can be used to decide from a set of available libraries with specific target optimizations. 
%Using a similar approach,  differential power analysis-based side channel attacks~\cite{kocher1999differential} may be mitigated by choosing the most appropriate cells or cell library (e.g., LVT vs. RVT vs. HVT) per cipher type.


\begin{figure*}[t]
   \includegraphics[width=\textwidth]{Images/Decision-Making Diagram (1).png}
   \centering
   \caption{General overview of decision making process for security-aware EDA using AI/ML/DL.}
   \label{fig:decisionmaking}
\end{figure*}



\paragraph{\textbf{Obfuscation for Black Box Designs during Logic Synthesis}}
Obfuscation is best implemented with complete structural and functional understanding of a circuit, but different levels of abstraction may present the challenge of having only one available. At the gate level, logic locking, as described in Section~\ref{par: dectuning, obfus}, may be viable, but the implementing party may also be restricted by their limited knowledge. Here again, a GNN seems capable of modeling the complex connections within the design, the competing needs to resist attacks, and narrowing down the most suitable implementation for balancing security and overhead. Ideally, the complete framework should provide locking options for each design and generate keys for a user discretely. Genetic algorithms have been applied to logic locking attacks like GenUnlock~\cite{chen2019genunlock}, where the evolutionary process is a black-box procedure overseen by an objective function. Conversely, this concept may be applicable to not only logic locking, but general obfuscation.




\subsubsection{Physical Design}
%Insert introductory text


\paragraph{\textbf{Security-aware Layouts and Tradeoff Modeling}} \label{subsubsec: eaprediction}

Invasive physical attacks are expensive to execute but difficult to protect against. Attackers resort to focused ion beam~(FIB) to extract an asset’s value by milling to its location in the IC layout, creating a metal contact to it, and probing the contact while the chip is in operation. There are two main sets of countermeasures proposed to combat probing attacks; the preventive strategy utilises active or analog shields, such as meshes, while the detection strategy checks for attacks by sensing any probing or editing and alerting the operators~\cite{wang2017}. To improve the effectiveness of active shields, an automated anti-FIB probing flow called iPROBE was proposed~\cite{Wang2019,osti_10174121}, see Fig.~\ref{fig:iprobe}. iPROBE uses ad hoc rules to determine the areas and metal layers where computer-aided design (CAD) tools should place shields to reduce ``exposed area''. For a physical IC, the exposed area (EA) metric (as described in \cite{shi2016layout}) is used to measure the design’s vulnerability to probing attacks. A larger EA means more flexibility with the expense that an attacker can probe without triggering contingencies. While iPROBE did improve EA while reducing overhead as compared to traditional shields, the security and overheads cannot yet be explicitly controlled by the designer. In other words, trial-and-error needs to be performed to make sure that constraints are met. To further boost efficacy of the anti-probing method described above, it may be possible to model the relationship between EA and power, timing and area with a multiple linear regression model or even DL. Then, iPROBE parameters could be chosen with security, area, power,~\etc{} in mind.

\begin{figure}[t]
\centering
%\includegraphics[width=0.85\columnwidth]{traceDefectsBorder.png}
\includegraphics[width=0.5\columnwidth]{Images/iProbev2.png}
\caption{iPROBE version 2 with protection for frontside and backside probing attacks~\cite{osti_10174121}. The light blue metal lines and darker blue metal lines form active shields that protect against frontside attacks (through top passivation and metal) and backside (silicon substrate), respectively. The metal lines sandwiched between the shields carry critical information that the attacker wants to probe. A FIB cut though an entire shield line of frontside/backside will be detected because the signal present on it will not match its counterpart in backside/frontside.}
\label{fig:iprobe}
\end{figure}


% •	E.g.) Porting of cryptographic and hardware security primitives to different technology nodes 
% The technology node (also process node, process technology or simply node) refers to a specific semiconductor manufacturing process and its design rules. Different nodes often imply different circuit generations and architectures. Generally, the smaller the technology node means the smaller the feature size, producing smaller transistors which are both faster and more power-efficient.
\paragraph{\textbf{Porting of Cryptographic and Hardware Security Primitives to Different Technology Nodes}}
Security-aware updates to designs are hardly ever direct ``out-of-box'' additions to devices. For integration of an IP or hardware security primitive, it is imperative that the design still fulfils its intended purpose. Selecting the most appropriate parameters for a hardware security primitive is one aspect, but another is porting it to a different technology node~\cite{keating_bricaud_2007}. Although technology nodes no longer categorically correspond to transistor gate length and half pitch, they nonetheless vary considerably with respect to manufacturing processes, design rules, noise sensitivity,~\etc{}~\cite{bagnato_indrusiak_quadri_rossi_2014}. These variations are noteworthy because they may disrupt the transferability of primitives. For example, an optimized PUF applied to an IC manufactured using the 28~nm process is not guaranteed to transfer to the 22~nm process due to factors like geometric variation and transistor type~\cite{keating_bricaud_2007}. The knowledge of process-specific parameters allows for assessment of the hardware primitive porting activity using ML. It is possible to use a classifier model as simple as an SVM to select the most suitable match between circuit and primitive without explicit knowledge of the design's functionality.


\paragraph{\textbf{Obfuscation for Black Box Designs during Physical Design}}
The physical design stage also presents opportunities for obfuscation to the designer with black box access using ML/DL. The current state-of-the-art in camouflaging is the covert gate approach~\cite{shakya2019covert}. Covert gates are inserted randomly into the design/layout, but a CNN or vision-based transformer can be incorporated to quantify the impact of insertion and ultimately identify the most viable gates to replace. 



% •	E.g.) Sensor optimization and : Why hide sensor optimization? Ask Dr. Forte 
% Add tamper, and side channel information.
\paragraph{\textbf{Anti-Counterfeit and Anti-Tamper Sensor Optimization}}
The scourge of IC counterfeiting continues to plague the semiconductor industry by flooding the consumer market with unauthorized, defective and inferior versions of original chips and designs. From as far back as 2006, electronic companies have missed out on \$100 billion of revenue due to counterfeiting~\cite{pecht2006}. The recent global chip shortage has created the avenue for these illegal devices due to demand exceeding current supply chain capabilities~\cite{leprince-ringuet_2021}. Recycled and remarked counterfeit ICs account for more than 80\% of the counterfeits sold worldwide~\cite{guin2014}. Hence, their detection has become a necessity to tackle IC counterfeiting. Recycled counterfeits are used chips fraudulently sold as new while remarked counterfeits are inferior chips sold as higher grades. 

Different sensors have been designed as a solution to these counterfeits, as seen in the work by by Zhang~\etal{}~\cite{zhang2014}. Their first of two proposed techniques uses frequency difference retrieved from paired ring oscillators (ROs) between an original and recycled chip to distinguish the two. RO frequency tends to degrade more with aging because the transistors in the RO gets slower with time~\cite{docking2003ro}. Guin~\etal{} also add anti-fuses and fuses for combating die and IC recycling (CDIR). Their RO-CDIR implementation is negative temperature instability-aware, which is valuable for flagging ICs with shorter usage~\cite{guin2014}. To date, the design of these sensors such as number of inverting stages, choice of threshold voltage, and overall structure are chosen in an ad hoc manner or through empirical means. Further, foundries do not always provide aging models to users. Both of these limits the age estimation of such sensors and their classification accuracy.


AI approaches, such as Bayesian optimization, would be preferable, especially for its ability to optimize black-box functions. Automating the optimization process will ultimately make it less-exhaustive.

Another source of hardware security issues is tampering. Once the device is physically compromised, it may leak on-chip information to the attacker. Hence, insertion of hardware Trojans may also be considered as tampering~\cite{tehranipoor2010}. One common example of tampering is FIB-based circuit edit, which allows an attacker to remove or bypass a security countermeasure~\cite{livengood_tan_hack_kane_greenzweig_2011}. Similar to recycling, sensors have been proposed to combat or detect tampering. A technique proposed by Liu and Kim uses logic-compatible embedded Flash (eFlash)-based tamper sensor built on an exposed floating gate (FG) structure to detect physical attacks~\cite{Liu2019}. Any change in charge stored on the exposed FG can be detected by this sensor. This includes humidity, high temperature, dust particles, chemicals, and electrostatic charges. A regression-based model or a neural network could fine-tune the configuration of such tamper sensors.
%Design space exploration for optimum placement, black box for sensitivity?


% Hiding sensor optimization: 
%Must review. Should be hiding after optimization to prevent the attacker from circumventing sensor
\paragraph{\textbf{Hiding Countermeasure Optimization}}
If an attacker is aware that a sensor has been deployed to detect a certain attack modality, the attacker may start by circumventing the sensor. For example, the attacker may apply the minimum possible mechanical force on the metal wires, or use a low intensity light source for a longer duration of time. Assuming maximum throughput possible, it is crucial to supplement successful optimization with robust defense. Hiding can dampen the signal accessible to the attacker. With limited knowledge of the sensor-IC design and operation, the designer could possibly rely on ensemble methods to find the most suitable hiding framework. The same sensors used to protect against tampering and detect counterfeits may also be vulnerable to side channel attacks. Since they are sensitive to changing parameters like voltage and frequency, they are prime targets for malicious parties. Sugarawa~\etal{} show that an attacker can reveal the internal state of a chip by observing how a sensor reacts to laser fault injection. The leakage leads to a feasible, non-invasive, probing attack. The sensor-type, the bit-flip detector, detects a short-circuit current induced by a laser fault injection~\cite{SUGAWARA201963}. Thus, it is advisable to supersede sensor optimization with robust hiding schemes; the ideal framework could combine both activities to boost resistance to side channel attacks. For example, if a noise generator is used as the default hiding mechanism, a simple regression model could predict the amount of noise required to achieve a lower signal-to-noise ratio (SNR). A more versatile system could have options like shielding in addition to noise generators, with decisions and settings also based on countermeasure optimization.



\paragraph{\textbf{Tuning EDA Parameters and Commands during Place-and-Route}}\label{subsubsec: dectuningpr}
%\paragraph{Placement-and-Routing}\label{par: dectuning, p&r}
At this stage of the design process, the manner of parameter tuning differs greatly from higher levels of abstraction. Improved P\&R decision-making means better chip area utilization, timing performance, and routability. A Pareto optimal solution may also be the best option, where significant parameter tradeoffs are required to achieve the best-possible design. Although most of the AI/ML applications at this stage have focused on obtaining complete design solutions, tuning parameters is still important for optimization. The authors of~\cite{karthik2018regplacement} use random forest (RF) regression techniques to tune guidelines and constraints for register placement. They are able to decide on the ideal location of each register and use that as seed placement for the entire design. One of its objectives is geared towards improved routing congestion, but a security-based implementation could address a countermeasure like obfuscation using different guidelines~\cite{karthik2018regplacement}.


 
% •	E.g.) Predict Trojan detection rates (dummy scan FF insertion, assertions, BISA, Split Manufacturing, run-time methods)
\paragraph{\textbf{Hardware Trojan Detection Rates during Layout}}
%2D vs 3D?
\textbf{Built-in self-authentication (BISA)} relies on the incorporation of functional filler cells into white spaces at the layout level to form built-in self-test (BIST) circuitry~\cite{xiao2013bisa}. The latter is designed to verify that no BISA cell is tampered with by an untrusted foundry. The possible failure of the BIST circuitry allows inserted Trojans to be detected. To reduce the risk of compromising BISA design during manufacturing, \textbf{split-manufacturing} can also be applied. On its own, split manufacturing cannot be used to detect Trojans, but the technique known as ``obfuscated BISA'' (OBISA)~\cite{shi2018obfuscated} combines both BISA and split-manufacturing. OBISA's ability to detect hardware Trojans can be predicted by training a machine learning model.







\subsubsection{Cross-Abstraction Applications}\label{crossabstraction}
%insert text

% Predict modeling area, power, timing as a function IP Protection (watermarking, FSM locking, camouflaging)
\paragraph{\textbf{Modeling Area, Power, Timing, and Security Impacts of IP Protection}} \label{subsubsec: ipprediction}

In general, design optimization problems have always been modeled based on area, power and timing; timing is used here because it directly relates to performance. Even at the HLS stage, ML implementations, like Pyramid~\cite{Makrani2019} have been used to predict optimal timing. There has also been work to predict area at both HLS~\cite{Zennaro2018} and logic synthesis~\cite{froemmer2020}. Deep-PowerX is a DNN-based dynamic power consumption minimization tool which exploits the power-area and delay-area relationships within a netlist~\cite{Pasandi2020}. Even at the placement and routing stage, timing prediction is possible using ML~\cite{Barboza2019}. 

One of the most significant threats to design integrity is IP piracy. The availability of a design to malicious parties gives way to overuse, modification, cloning, overproduction and/or reverse engineering. There are various defense-centered modifications available to an engineer at various stages of the IC design cycle, and ideas from ML-based optimization can be applied to them. 
%DNN used in Deep Power-X predicts error rates at primary outputs
\subparagraph{IP Watermarking} A watermark is a specific modification of an IP core that allows it to be uniquely identifiable, which is useful for piracy detection. However, IP core watermarking in general must never alter the functionality of the design~\cite{Chang2016watermark}. One popular method of watermarking is the the don't-care condition based technique. It involves adding function blocks with unspecified input combinations to the original design. Their outputs can be forced and used to verify the authenticity of a circuit~\cite{Dunbar2015SatisfiabilityDC}. However, additional logic may mean area, timing and power overhead. To hasten the design cycle, these overhead metrics must be readily available to a designer. If a trained algorithm can accurately model and predict these values, the design house would be able to ascertain the viability of a specific watermarking scheme, like the don't-care condition based method.

\subparagraph{Hardware Obfuscation}\label{par: dectuning, obfus} Hardware obfuscation is used to actively protect IP and has been applied at all major design stages preceding fabrication and assembly. It is intended to obscure an original design to prevent IP piracy and reverse engineering. Hardware obfuscation also addresses IP overuse and hardware Trojan insertion. 

The set of approaches that can be implemented until the DFT stage are typically \textbf{keyed} approaches. These techniques attempt to prevent black box use by key gates/inputs. One common example is \textbf{logic locking}, which hides the functionality and the implementation of a design by inserting additional gates (``key gates'') into the original netlist. The circuit will only function correctly if the acceptable inputs or keys are provided to the key gates~\cite{Yasin2020}. The additional gates must provide low overhead and be usable for larger designs. A significant challenge, however, has been making logic locking scheme secure against the entire suite of oracle-based attacks (e.g., SAT~\cite{subramanyan2015evaluating}, AppSAT~\cite{shamsi2017appsat}, key sensitization~\cite{rajendran2012security},~\etc{}.) and oracle-less attacks (e.g., desynthesis~\cite{massad2017logic}, signal probability skew~\cite{yasin2017security},~\etc{}.). The former use an unlocked chip as an oracle to non-invasively derive its key while the latter operate solely on the netlist. Preventing oracle attacks implies that the time to recover the key should be prohibitively high for an attacker. Recently, ML has been used to predict the obfuscation strength in terms of the predicted time taken to de-obfuscate an obfuscated circuit using the SAT attack. Chen~\etal{}~\cite{chen2020} demonstrate this using a GCN. They combine graph structure with gate feature by using an enhanced graph convolutional operator named ICNet. The features employed are divided into the graph structure, which describes connections, and gate features, including gate mask and gate type. While this approach has only been applied to predict SAT attack time, it can nonetheless be used to predict resistance to other oracle attacks. Recently, oracle-less attacks such as SAIL~\cite{chakraborty2018sail} have employed ML to recover the original (unobfuscated) netlist by reverse engineering logic synthesis rules.

Another key-based countermeasure that can be considered is FSM locking~\cite{chakraborty2009harpoon}. FSM locking adds extra states into the FSM of an IC design. The correct ``key'' is the right sequence of state transitions, which guarantees non-erroneous functionality. The additional states are materialised by FFs with their corresponding combinational logic. Active hardware metering~\cite{alkabani2007active}, a version of FSM locking, creates boosted finite state machines (BFSMs) from the new states. At this stage, it would be imperative to be able to predict the overhead created by the added states. This is because the design house sends the verified netlist to the untrusted foundry to create PUFs (challenge-response pairs) from the fabrication process variation. This may introduce additional overhead that could affect overall functionality. Depending on the complexity of the circuit, either a regression model or a DNN may suffice.

The \textbf{keyless} variety of obfuscation does not require keys, and cannot affect functionality. The desire is to conceal design intent. Without some form of obfuscation, a malicious party can either copy an IP or seek and exploit design vulnerabilities using reverse engineering. The most noteworthy example of keyless obfuscation is \textbf{IC camouflaging}~\cite{chow2012camouflaging}, which replaces original gates with ``camo gates'' which are difficult to discern by pattern recognition. It is worth noting, however, that most camouflaging techniques can be ``mapped'' into logic locked circuits~\cite{yasin2015transforming} where the above oracle attacks are quite effective~\cite{el2015integrated}. Hence, the prediction schemes mentioned above for logic locking may also apply to camouflaging. Further, the replacement of gates with camo gates to facilitate camouflaging will almost always alter power consumption and area. With the right set of features extracted from a report (HLS report), a trained regression model could predict the parameter values with near-perfect accuracy. There is evidence of this in other EDA applications. For example, Zennaro~\etal{} combine an RTL generation framework with ML algorithms to estimate the area of the final design based on the features of an abstract specification. They retrieve the number of configurable logic blocks (CLBs) information from synthesised RTL design reports created from an automation framework. They mainly use a multilayer perceptron (MLP), but also experiment with random forests (RF) and gradient boosting (GB)~\cite{Zennaro2018}.

Another popular keyless approach is \textbf{split manufacturing}~\cite{imeson2013securing} where a design is split, each part is fabricated at one or more untrusted entities, and a trusted entity puts them together. Split manufacturing can have significant overheads and security concerns (e.g., proximity attacks~\cite{magana2017proximity}) if P\&R is performed poorly. Ad hoc and linear programming approaches to perturb P\&R~\cite{wang2018cat} and/or split designs~\cite{shi2018obfuscated} have met with some success, but can likely be improved further through the incorporation of AI-based modeling and prediction.



% •	E.g.) Predict side channel resistance (hiding and masking schemes)
\paragraph{\textbf{Side Channel Attack Resistance}} \label{subsubsec: sidechannelresist}
Side channel leakage allows an attacker to break cryptographic systems. Signals that a cipher's implementation inadvertently emits allow for systematic extraction of underlying information. Examples include instantaneous power consumption, timing/delay, and electromagnetic emissions. Whether the attacker targets the understanding of device operation (simple) or uses leakage information to correlate data values (differential), there are generic countermeasures to reduce the effect of side channel leakage~\cite{markowitch_2011sca}. A high signal-to-noise ratio~(SNR) implies the availability of more meaningful leakage information. \textbf{Hiding} countermeasures reduce the SNR by either dampening the signal with low power designing and shielding, or flooding the leak-prone areas with noise using noise generators~\cite{levi2020ask}. To measure the value of hiding on a design, a predictive, regression-based model could provide an accurate percentage reduction in side-channel leakage. An obvious feature would be the tuning of the technique used. 

Another available countermeasure is \textbf{masking} which seeks to remove the correlation between input data and side-channel leakage ~\cite{prouff_2013_masking}. Unlike hiding, masking is applied at the algorithmic level with logic gates. Nonetheless, higher order side-channel analysis allows an attacker to bypass the routine masking schemes. A higher order masking may be employed but it may require significant overhead~\cite{prouff2009}. 
In order to evaluate the effectiveness of masking, various types of AI and ML algorithms have been employed to accomplish (a) the assessment of side-channel resiliency against a specific attack~\cite{picek2021sok}, and (b) the full leakage assessment methodology~\cite{moos2021dl}. 
However, both of these evaluation techniques need the actual ASIC or a correctly-programmed FPGA, as well as special equipment to be performed cf.~\cite{arribas2018vermi}. 
To overcome these obstacles, another line of research has been pursued, which is devoted to (1) theoretical conditions for a design to be SCA-resistant~\cite{barthe2015verified,coron2018formal,bloem2018formal} or (2) model the implementation for simulating its behavior~\cite{bertoni2017methodology,reparaz2016detecting} in the pre-silicon steps. 
In the first category, AMASIVE framework~\cite{zohner2012,huss2013amasive} can be mentioned that identifies hypothesis functions for leakage models cf.~\cite{buhan2021sok}. An example from the second class is VerMI, which is a verification tool in the form of a logic simulator that checks the properties of a class of masking methods (threshold implementation)~\cite{arribas2018vermi} at both algorithmic and implementation levels. 
Nevertheless, at this level of abstraction,~\ie{} pre-silicon, AI techniques have not found direct applications yet. Perhaps, the most straightforward way of incorporating such a technique can be imagined to examine whether the conditions for SCA-resiliency are fulfilled (the first category). 
%With the right features and a well-designed GNN, a designer could know how well masking works. A good template to follow would be the Adaptable Modular Autonomous Side-Channel Vulnerability Evaluator~(AMASIVE) framework~\cite{zohner2012,huss2013amasive} which autonomously identifies side-channel weaknesses in a design by highlighting design-specific vulnerabilities and exploiting them using an adaptable attacker model. 

%Placement and routing tool for side channel
Yet another step further, Ma~\etal{} presented a security-driven placement and routing tool to protect designs against EM side-channel attacks~\cite{CADSec2020} that attempts to break the balance of signal delays by register reallocation under the condition of layout constraints. The CAD-based tool, named CAD4EM-P, uses register reallocation and wire length adjustments to reduce the data dependency of EM leakage with acceptable area and power overheads~\cite{CADSec2020}. Opportunities to improve the effectiveness and efficiency of this approach can rely on more advanced forms of ML-for-prediction. For example, a graph neural network (GNN) can replace the graph-based algorithms that are the basis of the original version. 


% •	E.g.) Predict fault injection tolerance (redundancy in time and/or space)
\paragraph{\textbf{Fault Injection Tolerance}}
In contrast to most SCA attacks, fault injection attacks involve an active adversary.
In other words, the adversary tries to observe a faulty behavior of the target device by forcing it to function outside of its specified operating range or feeding it undefined data. 
For example, an attacker can cause erroneous operation of the target platform by tampering with the supply voltage (\aka{} voltage glitching), modifying the clock signal's frequency (a.k.a glitching), or flipping bits in the memory using a laser beam~\cite{bar2006sorcerer}.
While most fault attacks require physical access to the victim device, recent studies have shown that in certain cases similar fault attacks can also be carried out remotely on a variety of systems~\cite{alam2019ram}.
Cryptographic devices and secure hardware have been the main targets of fault injection attacks. 
For example, an adversary could inject faults into an FSM implemented on a hardware platform to bypass authentication states and obtain unauthorized access to security-sensitive states.
On the other hand, an adversary may be able to extract the secret key by injecting faults into a cryptographic implementation and applying mathematical tools, like Differential Fault Analysis (DFA), on faulty generated ciphertexts.

Several protection/detection-based countermeasures have been proposed to mitigate the vulnerabilities of circuits against fault attacks.
While device-level countermeasures can be effective against fault injection attacks, the cost and extra manufacturing steps make the algorithmic and circuit-based countermeasures more attractive.
EDA tools can be deployed to improve the circuits' resiliency for such countermeasures.
However, conventional countermeasures are generic and create high overhead in terms of area and power.
Several protection/detection-based countermeasures have been proposed to mitigate the vulnerabilities of circuits against laser fault injection~(LFI) attacks.
While physical countermeasures, such as tamper-proof packaging and light sensors, can be effective, the cost and extra manufacturing steps make the algorithmic and circuit-based countermeasures more attractive.
For such countermeasures, EDA tools can be deployed to improve the circuits' resiliency.
However, conventional countermeasures are generic and not tailored to specific fault injection techniques.
For instance, by using triple-modular redundancy~\cite{lyons1962use}, error-detection/correction codes~\cite{karpovsky2004new,sunar2007sequential,tomashevich2014protecting, neumeier2012punctured}, and MAC tags/infective computation~\cite{CAPA,MandM}, the circuit becomes more resilient in general.
In these cases, however, depending on the capabilities of the adversary and how these countermeasures are synthesized, placed, and routed, they can still be bypassed by powerful fault attacks.
AI/ML can support creating circuit netlists and layouts during the design phase that are more resistant to fault injection attacks by taking the physical models of fault attacks into account.
For instance, by considering fault propagation together as a new feature, the impact of fault resilient placement and routing on security and overhead can be predicted.



% •	E.g.) Predict increase in vulnerabilities across design abstractions, ports to different PDKs or FPGAs 

\paragraph{\textbf{Vulnerabilities Across Design Abstractions and/or PDKs}}
There is evidence that designs become more prone to certain security vulnerabilities as they move across different levels of abstraction. One example provided in \cite{jiang2018} presented a timing side-channel vulnerability introduced during HLS to produce an optimized RTL representation. Another pointed out fault-injection vulnerabilities after logic synthesis due to FSM encoding styles and newly generated don't-care states~\cite{nahiyan2019}. It is important to have foreknowledge of these potential risks as they develop during the EDA process. This is possible  with predictive algorithms. In one instance, the data flow graph representation of the RTL could be combined with features from the HLS report to produce a GNN capable of identifying less-secure design areas. 
This may also apply to porting designs across different process design kits~(PDKs). The available gate sizes are discrete values which are usually specific to the underlying technology. Process variations may introduce parametric alterations which could make a device more susceptible to malicious parties. For this scenario, PDK electrical and design rules are possible input features for the same GNN described above. As the solution space scales exponentially with respect to the size of the netlist, gate sizing algorithms integrated into EDA tools rely on either heuristics or analytical methods, which leads to sub-optimal sizing solutions. To combat this shortcoming,~\cite{lu2021rl} has demonstrated the feasibility of applying RL algorithms equipped with GNNs that encode design and technology features. 


% E.g.) Decide which benchmarks to use when evaluating an EDA tool
\paragraph{\textbf{Benchmark Selection for Security-Aware EDA Tool Evaluation}}\label{subsubsec: benchselection}
One additional optimization activity that may easily be overlooked is the evaluation of EDA tools used during the IC design process. Companies and research groups that develop EDA tools constantly update features to enhance their output. In order to properly target specific problem areas, the testing process must involve specific benchmarks. For example, if a designer intends to assess the scalability of the tool, the most important requirement for the test benchmark would be its size. If more nuanced conditions must be met, an automated method would make this process faster and more efficient. Succinct features of a benchmark and a tool's problem area in a DNN can determine the most suitable sample for testing. 

In the area of hardware security, benchmarking has played a critical role in development and comparison of hardware Trojan detection schemes~\cite{shakya2017benchmarking} and recently in de-obfuscation~\cite{amir2018development,tan2020benchmarking,amir2020adaptable}. Thus far, however, none of these benchmarking activities have explicitly incorporated AL/ML. 
 
 

 



\begin{figure*}[t]
   \includegraphics[width=\textwidth]{Images/Performance Prediction.png}
   \centering
   \caption{General overview of performance prediction process for security-aware EDA using AI/ML/DL.}
   \label{fig:performanceprediction}
\end{figure*}





\begin{figure*}[t]
   \includegraphics[width=0.85\textwidth]{Images/Black Box DSE.png}
   \centering
   \caption{General overview of black box optimization and design space exploration process.}
   \label{fig:blackbox}
\end{figure*}








\subsection{\textbf{Assimilation of Security Rules into Electronic Design Automation}}\label{aieda}
The incorporation of ML/AI into EDA describes replacing traditional heuristics with deep learning and AI-based decision-making policies that integrate the above steps (decision making, performance prediction, and optimization) into a single EDA framework. This will ultimately lead to a custom-based EDA pipeline based on the specific design and/or security application rather than relying on generic, somewhat-archaic EDA tools. Unlike  Section~\ref{subsec: blackbox}, the design space may stretch beyond what a designer has at their disposal. A valuable point to make is the possibility of utilizing a trainable decision-making policy in contrast to exploring the available decisions. The use of AI/ML almost guarantees more efficient results with shorter runtimes. There is budding research within the IC design community to incorporate learning-based tools into the EDA pipeline. 
The OpenROAD project is a DARPA-funded initiative which seeks to solve EDA cost and turnaround time. The goal is to complete the design process without performace, power or quality tradeoffs using ML, cloud-based optimization and other techniques~\cite{ajayi2019openroad,connor_2018}. Their work so far has incorporated problem-specific tools like ioPlacer for fast and scalable input/output pin assignment~\cite{bandeira2020ioPlacer}, TritonCTS for clock tree synthesis~\cite{Han2020OptimalGH} and RTL-MP for macro placement using RTL information and clustering~\cite{kahng_varadarajan_wang_2022}. A team of researchers at Google also presented a floorplanning tool for the physical design stage that can successfully place macro blocks using deep RL~\cite{Mirhoseini2021AGP}. Its results demonstrated improvement over traditional manual efforts across performance, power consumption and area, and allowed its application to a recent tensor processing unit (TPU) product.

Unfortunately, very little work has been done to utilize learning models to make designs security-aware at every major stage. With AI/ML firmly established in the pipeline, design optimization and security could be combined. Design-specific EDA will make extraneous steps obsolete and ultimately reduce the time-to-market for ICs. Table~\ref{tab: aieda} highlights the areas of interest for each major design stage.


%Add table to show various major steps and rules incorporated
%Common Security schemes with applicable design stages and machine learning algorithms used
\begin{figure*}[t]
   \includegraphics[width=\textwidth]{Images/AIEDA (1).png}
   \centering
   \caption{General overview of AI-assisted EDA. The emphasis is on direct application to EDA.}
   \label{fig:aieda}
\end{figure*}


% % •	Identifying and incorporating security rules/properties at all steps

% \subsubsection{\textbf{Assimilation of Security Rules into the Design Process}}

The manufacture of secure ICs must begin with embedding of security rules at major steps of the design process. This encompasses the acts of identifying, assessing and incorporating prerogatives and properties within specific stages. All design steps follow defined rules during their series of actions on the input design~\cite{khwaja1997edarule}. For example, during logic synthesis, minimization may occur by combining gate terms where applicable to reduce circuit size~\cite{brayton1990logicsyn}. Even design constraints can be described as rules because they define the behavior of the design at each point of usage. In the same vein, it is necessary to apply security rules as rigorous requirements throughout the entire design sequence. 

Efforts to support such assimilation are starting to grow. For example, the Hardware Common Weakness Enumeration Special Interest Group (HW CWE SIG)~\cite{CWE_MITRE} consists of researchers and representatives from organizations operating in hardware design, manufacturing, and security who interact, share opinions and expertise, and leverage each other’s experiences in defining hardware security weaknesses and identifying them with analysis tools. However, the current initiative is manual and quite subjective. Data-driven and AI-based approaches could make this less tedious and more objective in nature.


%Table

 



% o	HLS/RTL (ASIC/FPGA)
% Obfuscation
% Masking
% Information flow security – automatic identification of assets and/properties in designs through ML/AI


\subsubsection{High Level Synthesis and Register Transfer Level}
The overall design of a circuit depends on the requirements stated in its specifications. Traditional execution of HLS results in an RTL description of the design, which is a better hardware-based representation of the intended IC. During the design process, it is difficult to ascertain certain features and how they may impact the entire circuit, but significant work has been done to mitigate this using ML~\cite{Makrani2019,Zennaro2018, Dai2018}. One noteworthy ML-based optimization framework combines a GNN with RL to predict design results and obtain optimal solutions under user-specified constraints and objectives like area and latency~\cite{wu2021ironman}. The security-aware designer can also leverage ML to anticipate and solve security problems that an IC is vulnerable to. Security rules at this early stage of the design process are less-tedious and reasonably-inexpensive to enforce.

Pre-synthesis obfuscation is applied to a design prior to the logic synthesis stage. Although the most prevalent techniques are used post-synthesis, there has been work done on this early stage method of obfuscation. Obfuscation can be implemented at the high level stage before conversion into RTL. One group uses MUXes driven by a locked controller units to create decoy connections~\cite{rajendran2015}. Exploiting the MUX's use of inputs and a control signal, only the correct control signals can unlock the design. The authors of \cite{Chakraborty2010} convert RTL code into control and data flow graph (CDFG) form, apply locking by superimposing an authentication FSM, and then return to RTL. Both applications may be deployed as security rules with deep learning-based execution. The CDFG form could be implemented as a GNN for optimum modeling of a design's complexity.

Masking to prevent differential power analysis (DPA) during a side channel attack is also possible at this level of abstraction. Konigsmark~\etal{} create an HLS flow which addresses side-channel leakage by inferring security critical operations from user-specified confidential variables in HLS input. Their modified framework rectifies imbalanced branches that pose easy attack targets, and changes functional units based on leakage potential~\cite{konigsmark2017}. This experiment could be the foundation for learning-based masking solutions to prevent SCA; it stands to be improved by feature-based rectification. 

It is important to verify that systems adhere to information flow security (IFS) policies, especially during the design phase. All assets flowing through the system must be identified; this is known as information flow tracking (IFT)~\cite{hu2021}. Achieving this at higher levels of abstraction reduces the effort required to rectify potential problems. One publication presents RTLIFT as a means of measuring all digital flows through RTL designs to formally prove security properties related to integrity, confidentiality and logic side channels~\cite{Ardeshiricham2017}. Perhaps its most impressive property is the ease of integration into the design flow. Intelligent decisions surrounding security policies means adaptability to different designs trade-offs such as the RL-based policy iteration to calculate digital flows and possibly flag irregularities~\cite{Ardeshiricham2017}. 



\begin{table}
\centering
\caption{Major IC design stages in EDA with security needs and possible applications of AI/ML.}
\arrayrulecolor{black}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|} 
\hline
\rowcolor[rgb]{0.361,0.769,0.769} {\cellcolor[rgb]{0.361,0.769,0.769}}        & {\cellcolor[rgb]{0.361,0.769,0.769}}              & {\cellcolor[rgb]{0.361,0.769,0.769}}                    & \multicolumn{2}{c|}{\textbf{AI/ML Algorithms Applicable}}            \\ 
\hhline{|>{\arrayrulecolor[rgb]{0.361,0.769,0.769}}--->{\arrayrulecolor{black}}--|}
\rowcolor[rgb]{0.361,0.769,0.769} \multirow{-2}{*}{{\cellcolor[rgb]{0.361,0.769,0.769}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.361,0.769,0.769}}c@{}}\\ \textbf{Design Stage}\end{tabular}}   & \multirow{-2}{*}{{\cellcolor[rgb]{0.361,0.769,0.769}}\textbf{Security Task}}            & \multirow{-2}{*}{{\cellcolor[rgb]{0.361,0.769,0.769}}\textbf{Design Type}} & \textbf{Suggested}         & \textbf{Implemented}                    \\ 
\hline
{\cellcolor[rgb]{1,0.859,0.604}}        & Obfuscated Design              & \multirow{3}{*}{ASIC, FPGA}          & RL      & GNN~\cite{rozhin_2021}                      \\ 
\hhline{|>{\arrayrulecolor[rgb]{1,0.859,0.604}}->{\arrayrulecolor{black}}-~--|}
{\cellcolor[rgb]{1,0.859,0.604}}        & Masking     &                   & GNN, GCN, RF               &                      \\ 
\hhline{|>{\arrayrulecolor[rgb]{1,0.859,0.604}}->{\arrayrulecolor{black}}-~--|}
\multirow{-3}{*}{{\cellcolor[rgb]{1,0.859,0.604}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{1,0.859,0.604}}c@{}}\textbf{High Level Synthesis and}\\\textbf{~Register Transfer Level}\end{tabular}} & Information Flow Security      &                   & RL      &                      \\ 
\hline
{\cellcolor[rgb]{1,0.859,0.604}}        & Obfuscated Design              & \multirow{4}{*}{ASIC, FPGA}          & GCN     & ~ ~ANN~\cite{Sisejkovic2021-challenge-logic-locking}            \\ 
\hhline{|>{\arrayrulecolor[rgb]{1,0.859,0.604}}->{\arrayrulecolor{black}}-~--|}
{\cellcolor[rgb]{1,0.859,0.604}}        & Masking     &                   & RL, GNN &                      \\ 
\hhline{|>{\arrayrulecolor[rgb]{1,0.859,0.604}}->{\arrayrulecolor{black}}-~--|}
{\cellcolor[rgb]{1,0.859,0.604}}        & Information Flow Security      &                   & GCN     &                      \\ 
\hhline{|>{\arrayrulecolor[rgb]{1,0.859,0.604}}->{\arrayrulecolor{black}}-~--|}
\multirow{-4}{*}{{\cellcolor[rgb]{1,0.859,0.604}}\textbf{Logic Synthesis }}                      & Side Channel Resistance        &                   & GNN     &                      \\ 
\hline
{\cellcolor[rgb]{1,0.859,0.604}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{1,0.859,0.604}}c@{}}\textbf{Device Sizing/ }\\\textbf{Technology Mapping}\end{tabular}               & Fault Tolerance                & ASIC              & Bayesian Optimization, DNN &                      \\ 
\hline
{\cellcolor[rgb]{1,0.859,0.604}}        & Crosstalk Mitigation           & \multirow{5}{*}{ASIC, FPGA}          &         & \begin{tabular}[c]{@{}c@{}}Logistic Regression~, \\XGboost~\cite{liang2020crosstalk} ~\end{tabular}  \\ 
\hhline{|>{\arrayrulecolor[rgb]{1,0.859,0.604}}->{\arrayrulecolor{black}}-~--|}
{\cellcolor[rgb]{1,0.859,0.604}}        & Anti-tamper layouts            &                   & GCN, RL &                      \\ 
\hhline{|>{\arrayrulecolor[rgb]{1,0.859,0.604}}->{\arrayrulecolor{black}}-~--|}
{\cellcolor[rgb]{1,0.859,0.604}}        & \begin{tabular}[c]{@{}c@{}}PDNs for anti-side channel \\and fault injection\end{tabular}                   &                   & GNN     &      Linear Regression~\cite{utyamishev2020power}                \\ 
\hhline{|>{\arrayrulecolor[rgb]{1,0.859,0.604}}->{\arrayrulecolor{black}}-~--|}
{\cellcolor[rgb]{1,0.859,0.604}}        & Anti-RE layouts                &                   & GCN                   &       CNN~\cite{zargari2021captive}               \\ 
\hhline{|>{\arrayrulecolor[rgb]{1,0.859,0.604}}->{\arrayrulecolor{black}}-~--|}
\multirow{-5}{*}{{\cellcolor[rgb]{1,0.859,0.604}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{1,0.859,0.604}}c@{}}\textbf{Floorplanning and}\\\textbf{~Physical Design }\end{tabular}}               & Custom eFPGA fabrics           &                   & RL      &                      \\ 
\hline
{\cellcolor[rgb]{1,0.859,0.604}}        & \begin{tabular}[c]{@{}c@{}}Test point insertion and pattern \\generation for Trojan detection\end{tabular} & \multirow{3}{*}{ASIC, FPGA}          & RF, GB  & RL\cite{pan2021atpg}     \\ 
\hhline{|>{\arrayrulecolor[rgb]{1,0.859,0.604}}->{\arrayrulecolor{black}}-~--|}
{\cellcolor[rgb]{1,0.859,0.604}}        & Information flow security      &                   & GNN, DNN,  RL    &                      \\ 
\hhline{|>{\arrayrulecolor[rgb]{1,0.859,0.604}}->{\arrayrulecolor{black}}-~--|}
\multirow{-3}{*}{{\cellcolor[rgb]{1,0.859,0.604}}\textbf{Testing and Verification }}             & \begin{tabular}[c]{@{}c@{}}Comparison of original \\specification to final design\end{tabular}             &                   & GNN     & NLP\cite{yu2021hw2vec}                      \\
\hline
\end{tabular}
}
\label{tab: aieda}
\end{table}

% Logic Synthesis (ASIC/FPGA)
\subsubsection{Logic Synthesis}
In general, logic synthesis has been extensively-researched under AI/ML~\cite{Neto2019LSOracleAL, pasandi2019approximate,Pasandi2020}. The RTL-to-gate level process provides viable data to train models that have mostly been used for design optimization. The conversion from behavioral level to the gate level is the bridge between a design idea and its generation because the specific logic functions are implemented from combinations of gates selected in a given cell library.



% Obfuscated at gate level: FSM Locking, revisit logic locking, available in hardware obfuscation book

At the gate-level, the first form of obfuscation which comes to the security-aware designer's mind is logic locking. With various methods available, there is little existing work using AI/ML. One proposed work that could be the baseline for future exploration is LeGO~\cite{alaql2021}. The authors point out that it can iteratively harden a design against a set of attacks. The framework begins by performing a simple key-based locking and continues with an iterative feedback process which considers a set of possible attacks to defend against~\cite{alaql2021}. The attacks are provided with corresponding countermeasures for integration. The rule selection algorithm, which uses prior knowledge from a database of mitigation rules, identifies the best protection to be applied for each key-bit against a specific attack. The "convergence point" occurs when all security issues are addressed~\cite{alaql2021}. The learning design could be improved with an RL-based policy iteration framework. With a suitable representation of the gate-level netlist and its features, there are many possibilities.


% Side channel resistance – distribution of side channel countermeasures: include masking, hiding~\etc{}.
% Information flow security


Similarly, in the quest for side-channel resistant designs, gate-level masking has been researched since the early 2000s. Masking is most ideal for implementation at this stage, because of the gate design's correlation to the physical design's functionality. In 2005, masked dual-rail pre-charge logic (MDPL) was proposed as a promising DPA-resistant logic style~\cite{Popp2005}. MDPL circuits are based on a standard cell libraries and have no routing constraints concerning the balancing of complementary wires. The dual-rail pre-charge property of MDPL specifically prevents glitches in the circuit. A more recent implementation uses a technique that combats the phenomena of glitches and early propagation using only cell-level “don’t touch” constraints~\cite{Leierson2014}. Their framework, a derivative of MDPL called LUT-Masked Dual-rail with Precharge Logic (LMDPL), can works for both FPGA or and ASIC designs. MDPL may be used as a rule-based template for masking gate-level designs. A GCN can be used to identify sections of the circuit that are vulnerable and would require MDPL implementation.


Information flow tracking at the gate level also serves to check adherence to security policies. The well-defined gate level information flow tracking (GLIFT) technique has been widely used to GLIFT used to design secure hardware architectures and detect security violations from visible timing flows. Hardware trojan dection has even been accomplished based on harmful information flows that point to sensitive information leakage and data integrity violation~\cite{nahiyan2017trojandetection}. From Fig.~\ref{fig:glift}, the RTL synthesis which produces the gate level representation is followed by standard cell augmentation with shadow logic gate. Design stage verification is the most suitable application of GLIFT to the EDA pipeline. The technique only checks for violation of IFS policies without addition of logic to the fabricated design. Once again, a GCN representation with sufficient features may be used to supplement, or even replace GLIFT.

\begin{figure*}[t] %replace with design stage verification
   \includegraphics[width=0.9\textwidth]{Images/Glift flow.png}
   \centering
   \caption{GLIFT workflow with standard cell and GLIFT libraries.}
   \label{fig:glift}
\end{figure*}




% Device Sizing and/or Technology Mapping (ASIC only)
% Fault tolerance


\subsubsection{Device Sizing and/or Technology Mapping}
For ASIC designs, device size is crucial to the success of a design. The targeted purpose of ASICs means even the slightest deviation from specified dimensions will result in a failed design process. The technology-mapping step converts internal representation and the optimized logic based on the designated technology library~\cite{kaufmann2008techmap}. The mapped netlist nodes are implemented with available components to optimize area, power and/or delay; the gates in a library are have pre-defined values for these parameters. RL is capable of further optimizing the entire design with regard to power, area and delay. Techniques for approximate logic synthesis (ALS) suffer from long execution time, which has been addressed in~\cite{pasandi2019approximate} by adopting RL-based strategies. 

Critical assets in devices may be compromised by taking advantage of errors from fault injection. Single event upsets (SEUs) affect sequential elements, while single event transients (SETs) arise from combinational logic~\cite{BOGAERTS2014250}. An SEU may lead to a single event latchup (SEL), which results in a high operating current, or a short circuit. Fault tolerance reduces the sensitivity of devices to particle or laser attacks that cause these events. Glitches can be used to progressively break cryptography schemes or disable internal protection mechanisms~\cite{giraud2010}. Redundant computation is one way of making designs impervious to upsets. It uses double computation (in time or space) with a final comparison; if the results from redundant computations do not match, the output of the encryption function is suppressed/randomized. Redundancy may cause increased area and power consumption, but methods like the one presented in~\cite{petrovic2012} show high tolerance with moderate overhead is possible. The optimization procedure can be refined using a Gaussian process to find the best trade-off value.


% Floorplanning and Physical Design (ASIC/FPGA)
% Crosstalk
% Power delivery networks for anti-side channel/fault
% Anti-tamper layouts
% Anti-RE layouts
% Custom eFPGA fabrics


\subsubsection{Floorplanning and Physical Design}
The floorplanning step formalizes the high level design established at the beginning of the process, and is followed by P\&R to connect all blocks such that they meet design criteria and constraints. After initial P\&R attempts, the design’s timing constraints are analyzed~\cite{martin_scheffer_lavagno_2016}. If unsatisfactory, the P\&R software in use tries different placements and signal routing to try to meet the designated constraints. Even outside academia, work has been done on automating floorplanning to benefit the physical layout. Researchers at Google modeled chip floorplanning as a reinforcement learning (RL) problem, and used a GCN representation of the design to optimize power, area and performance~\cite{Mirhoseini2021AGP}. 



Design scaling from a technology process may reduce spacing between adjacent interconnects; the resulting increased coupling capacitance between wires causes crosstalk~\cite{zhou1998crosstalk}. The affected signal's value may either change, or have delayed signal transition. False clocking, where a clock changes states unintentionally, may also occur~\cite{terapasirdsin2010crosstalk}. Good signal integrity is necessary for optimum functionality of an IC~\cite{green1999}. Large signal-integrity problems may cause intermittent success or complete system failure. To address crosstalk, the design tool must be able to measure its value. The authors of \cite{chang2006} find a closed form expression of crosstalk using a number of wires. With accurate metrics, a linear regression model coupled with the RL method applied in~\cite{Mirhoseini2021AGP} could address crosstalk expeditiously.


Side channel leakage is one of the results of the nature of an IC's power distribution network (PDN). The PDN is responsible for the supply of stable voltage and power to each functional component of the circuit~\cite{martin_scheffer_lavagno_2016}, but it may also inadvertently introduce side-channel leakages throughout the design~\cite{zhang2020pdnsca}. The growing complexity of devices introduces sophisticated PDNs with the potential to allow successful side-channel attacks or fault injection. To improve the security of a design, it is important to use ML to build on existing work on this topic. PowerScout is a framework geared towards evaluating side-channel vulnerabilities by modeling possible attacks to improve PDN designs~\cite{zhu2020}. It can effectively predict leakage strength and also identify fault injection soft spots. The side channel and fault injection attacks are modeled using non-learning based design space exploration. A decision tree, or an MLP could predict these with the same parameters being extracted. There may also be promise in modeling the PDN using a graph-based network and optimizing leakage-prone nodes for the physical design.


Anti-tamper designs are meant to deny an adversary’s opportunity to monitor or affect the correct operations of an IC. At the layout level, one CAD assessment technique allows a designer to gauge a designs susceptibility to frontside probing attacks~\cite{Wang2019}. The assessment is performed by varying attack parameters (FIB aspect ratios and angles), shield parameters (layers and shape) and the assets under attack (keys, buses,~\etc{}.). Two of the most useful aspects of the paper are the exposed area (EA), which is free to probe without impacting transmission, and shield structure taxonomy, which is a set of documented shield patterns~\cite{Wang2019}. Based on the attack parameters, EA and the shield taxonomy, an RL model could help recommend the best shield design for a layout.


At the layout level, IC camouflaging is a EDA engineer's most suitable option to prevent successful RE. The camouflaged layout is a functional replica of the original design with camo gates (See ~\ref{subsection: decisionmaking}. A novel framework for secure layout generation could focus on generating camo gates using GANs. Recommendations for camouflage points on an IC can be modeled using a GCN or a CNN.



The embedded FPGA (eFPGA) is an IP core integrated into an ASIC that offers the reprogramming flexibility of FPGAs without their overhead costs. They are added to systems which require frequent updates; by adding their fabric to an SoC or ASIC, teams are able to modify applications seamlessly. One security evaluation in \cite{Bhandari2021} points out that eFPGAs can contribute to SAT attack resilience. The eFPGAs have combinational loops that a specific cyclic SAT solver like CycSAT~\cite{zhou2017} cannot solve. Increasing attack difficulty can be considered when creating eFPGA fabrics at the physical design stage. The incorporation of a policy-based model that incorporates this into an ASIC design could improve security considerably.



% Testing and Verification (ASIC/FPGA)
% Test point insertion and pattern/generation for Trojan detection
% Information flow security checking
% NLP to match original spec and final design
\subsubsection{Testing and Verification}

As an IC reaches its physical state, the designers must implement design testing and verification. It is important to point out that most major design stages reach completion via some form of verification step~\cite{wang2009electronic}. For example, the logic synthesis step utilizes an RTL and gate level netlist verification procedure to guarantee functionality retention of the gate level design~\cite{martin_scheffer_lavagno_2016}. Testing and verification combined ensure that an IC has maintained original specifications and functionality throughout the design process. For physical testing, the two most significant options are wafer level testing and package level testing~\cite{perry_2007}. 



% Test point inserton and ATPG for predicting trojans. 


Design for Testability (DFT) is a technique employed in designing ICs for the purposes of reducing test costs and associated time. A very common technique for DFT is scan-chain insertion; regular FFs in the design are replaced with scan FFs. ATPG is a test methodology used to identify faulty behavior(s) in circuits due to design defects. The goal of ATPG is to create a set of test patterns that achieve a desired test coverage, TC, and fault coverage, FC, through fault simulation~\cite{hardware2011}. ATPG and formal methods have been researched for Trojan detection, but most do not consider partial-scan instances of a third-party IP (3PIP). The authors of~\cite{cruz2018} generate a set of constraints using the model checker to facilitate directed test generation using ATPG tool. A constraint generation procedure uses model checking to produce a set of signal traces. A test vector generation method then uses ATPG with the design, rare nodes and signal traces to produce a set of test vectors for activating each rare node~\cite{cruz2018}.


%Information flow security? Rewrite, Design space exploration for decisions circuit modeling, DFG, RL
At the verification stage of the design flow, IFT can be executed using static or dynamic techniques. Static techniques assess the design's compliance with security policies using simulation, formal verification, emulation or virtual prototyping. They are applicable within the EDA pipeline, and are removed when verification is completed~\cite{hu2021}. Due to the unique goals of each specific static technique, AI/ML can be added to decrease resource usage, and improve results. For hardware security simulation, levels of abstraction like gate level and RTL are viable. As described in logic synthesis, graph-based networks are ideal solutions. The simulation process links security labels to signals. Formal verification guarantees proof of security for the desired properties, but it is known to have scaling issues~\cite{hu2021}. The large design state space of complex systems requires a policy-based learning solution which RL provides. Emulation can perform hardware-software co-verification, using FPGA emulation servers. Learning-based models could make these servers more robust to even detect software vulnerabilities that impact hardware. The abstract models of hardware components created by virtual prototyping can be tested a different RL-based approach. If the policy used is geared towards creating security problems while verifying software, the designer becomes aware of impending problems. Dynamic techniques use dedicated hardware to track information flow during runtime. A neural network could validate results to predicting flow inconsistencies.


Furthermore, Natural language processing (NLP) can be applied to circuit designs at different levels of abstraction. One of the most promising bridges to this is HW2VEC, a graph learning tool to extract graph representations from a hardware design in either RTL or gate level~\cite{yu2021hw2vec}. It is divided into two main parts: a HW2GRAPH stage which converts the design to a graph while retaining structural information, and GRAPH2VEC which converts the graph into Euclidean-based embeddings. GRAPH2VEC is just one of a number of graph-to-vector-embedding algorithms that utilizes concepts from the skipgram word embedding model~\cite{narayanan2017graph2vec}. The resulting vector representation may be applied with measures of similarity, like cosine similarity, to verify designs. If HW2WEC can be leveraged at physical design stages, the final IC product can be verified for structural authenticity.
 


